RecTen: A Recursive Hierarchical Low Rank Tensor Factorization Method to Discover Hierarchical Patterns in Multi-modal Data

How can we expand the tensor decomposition to reveal a hierarchical structure of the multi-modal data in a self-adaptive way? Current tensor decomposition provides only a single layer of clusters. We argue that with the abundance of multimodal data and time-evolving networks nowadays, the ability to identify emerging hierarchies is important. To this effect, we propose RecTen, a recursive hierarchical soft clustering approach based on tensor decomposition. Our approach enables us to: (a) recursively decompose clusters identified in the previous step, and (b) identify the right conditions for terminating this process. In the absence of proper ground truth, we evaluate our approach with synthetic data and test its sensitivity to different parameters. We also apply RecTen on five real datasets which involve the activities of users in online discussion platforms, such as security forums. This analysis helps us reveal clusters of users with interesting behaviors, including but not limited to early detection of some real events like ransomware outbreaks, the emergence of a blackmarket of decryption tools, and romance scamming. To maximize the usefulness of our approach, we develop a tool which can help the data analysts and overall research community by identifying hierarchical structures. RecTen is an unsupervised approach which can be used to take the pulse of the large multi-modal data and let the data discover its own hidden structures by itself.

==> 009-Acknowledgment.tex <==
\section{Acknowledgment}
\label{sec:Acknowledge}

%\thanks {This work was supported by  DHS ST Cyber Security (DDoSD)  HSHQDC-14-R-B00017 grant and the Bourns College of Engineering at UC Riverside}
%Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the funding parties.
 {%The authors thank the anonymous reviewers for their useful comments.
This material is based upon work supported by DHS ST Cyber Security (DDoSD)  HSHQDC-14-R-B00017 grant. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of 
%the National Science Foundation or other 
the funding institutions.}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> arxiv-RECTEN (2)/000-dfn.tex <==


\newcommand{\risul}[1]{{\bf {\textcolor{green}{Risul:}}{\textcolor{blue}{#1}}}}

\newcommand{\rismi}[1]{{\bf {\textcolor{green}{R+M:}}{\textcolor{red}{#1}}}}

\newcommand{\miii}[1]{{\bf  {\textcolor{blue}{MF:}}{\textcolor{red}{#1}}}}

 \newcommand{\miok}[1]{{\bf {\textcolor{OliveGreen}{#1}}}}

\newcommand{\hide}[1]{}
%\newcommand{\comment}[1]{{\tiny #1 }}
\newcommand{\semihide}[1]{{\tiny #1}}
\newcommand{\changed}[1]{{\textcolor{blue}{#1}}}
%\newcommand{\reminder}[1]{{\textcolor{red}{#1}}}
\newcommand{\proofApp}[1]{{\emph{\bf Proof of #1.}}}
% \newcommand{\makeclean}{
\newcommand{\mkclean}{
    \renewcommand{\reminder}[1]{}
    \renewcommand{\comment}[1]{}
    \renewcommand{\semihide}[1]{}
    \renewcommand{\changed}[1]{}
}


\newcommand{\RelThreads}{$R_t$}
 % most relevant threads  based on their relevance socre

\newcommand{\method}{{\tt HackerChatter}}
\newcommand{\source}{O}
\newcommand{\destination}{D}
\newcommand{\node}{\ensuremath{v}}
\newcommand{\edge}{\ensuremath{e}}
\newcommand{\graph}{\ensuremath{\mathcal{G}}}
\newcommand{\length}{\ensuremath{{l}}}
\newcommand{\prob}{\pi} 
\newcommand{\error}{e}
\newcommand{\fun}{f}
\newcommand{\loc}{\lambda}
\newcommand{\outdeg}{d_{out}}
\newcommand{\base}{b}
\newcommand{\dist}{\delta}
\newcommand{\ratio}{\rho}
\newcommand{\extrad}{\alpha}
\newcommand{\nodec}{\nu}
\newcommand{\pvalue}{p-value}
\newcommand{\mean}{average}
\newcommand{\std}{standard-deviation}
\newcommand{\ba}{\beta_{0}}
\newcommand{\bb}{\beta_{1}}
\newcommand{\bc}{\beta_{2}}

\newcommand{\HH}{Heavy-Hitters\xspace}
\newcommand{\CS}{Consumers\xspace}
\newcommand{\HP}{High Producers\xspace}
\newcommand{\AP}{Average Producers\xspace}
\newcommand{\LP}{Low Producers\xspace}
\newcommand{\PR}{\textit{Producers}\xspace}
\newcommand{\Rho}{\mathrm{P}}
\newcommand{\expnumber}[2]{{#1}\mathrm{e}{#2}}

\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}



\newcommand{\OffComm}{OffensiveCommunity\xspace}
\newcommand{\OffCommShort}{OffensComm.\xspace}
\newcommand{\HTS}{HackThisSite\xspace}
\newcommand{\WSForum}{WildersSecurity\xspace}
\newcommand{\Ash}{Ashiyane\xspace}
\newcommand{\WSShort}{WildersSec.\xspace}
\newcommand{\Ethical}{EthicalHackers\xspace}
\newcommand{\EthicalShort}{EthicHacks\xspace}
\newcommand{\darkode}{Darkode\xspace}


\newcommand{\TT}{{\em Hacks}\xspace}
\newcommand{\PS}{{\em Services}\xspace}
\newcommand{\AN}{{\em Alerts}\xspace}
\newcommand{\AG}{{\em Experiences}\xspace}

\newcommand{\MV}{{\em Malware - Virus}\xspace}
\newcommand{\HA}{{\em Hack - Account}\xspace}
\newcommand{\TG}{{\em Tutorial - Guide}\xspace}
\newcommand{\SB}{{\em Sell - Buy}\xspace}
\newcommand{\AV}{{\em Attack - Vulnerability}\xspace}
\newcommand{\VG}{{\em Video - Game}\xspace}
\newcommand{\CC}{{\em Credit Card}\xspace}





% \newcommand{\myalg}{RKEA\xspace}
% \newcommand{\myalgFull}{{\bf R}ecursive {\bf K}eywords {\bf E}xtracting  {\bf A}pproach\xspace}

\newcommand{\seedMethod}{Initialization via domain adaptation\xspace}



\newcommand{\seedMethodAcro}{IDA\xspace}

%\newcommand{\WordsFreq}{\textit{WordsFreq}\xspace}
\newcommand{\WordsFreq}{\textit{TextInfo}\xspace}
\newcommand{\IPP}{\textit{DecimalVal}\xspace}
\newcommand{\Mixed}{\textit{Mixed}\xspace}
\newcommand{\Cocluster}{\textit{Co-Cluster}\xspace}

\newcommand{\extUserWord}{\textit{ContextInfo}\xspace}
\newcommand{\extUserWordlong}{Contextual Information\xspace}


\newcommand{\PostTextlong}{Text information of the post\xspace}   %% FIRST CAPITAL
\newcommand{\postTextlong}{text information of the post\xspace}
\newcommand{\postText}{\textit{PostText}\xspace}
 

\newcommand{\mfal}[1]{{\bf{\textcolor{blue}{MF:}}{\textcolor{red}{#1}}}}
\newcommand{\mrem}[1]{{\bf{\textcolor{green}{\xspace#1}}}} 

%\newcommand{\mfal}[1]{}

\newcommand{\idenp}{Identification\xspace}
\newcommand{\classp}{Characterization\xspace}

\newcommand{\crosstrain}{cross-training\xspace} %% WE want this to imply learning from another forum, when we lack seed data

\newcommand{\cseed}{Cross-Seeding\xspace} 

\newcommand{\cporting}{Basic\xspace} %% name for when we just tranfser the classifier

\newcommand{\kwords}{$W$\xspace}
\newcommand{\kwordsDef}{Word-Range\xspace}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% unquote the below to remove reminders
\newcommand{\eatreminder}{\renewcommand{\reminder}{\hide}}
%\eatreminder






==> arxiv-RECTEN (2)/001-abstract.tex <==

\begin{abstract}
How can we expand the tensor decomposition to reveal a hierarchical structure of the multi-modal data in a self-adaptive way? 
Current tensor decomposition provides only a single layer of clusters.
We argue that with the abundance of multi-modal data and time-evolving networks nowadays, the ability to identify emerging hierarchies is important. To this effect, we propose \algo, a %parameter-free 
recursive hierarchical soft clustering approach based on tensor decomposition. 
Our approach enables us to: (a) recursively decompose clusters identified in the previous step, and (b) identify the right conditions for terminating this process. 
% We argue that it is not easy to fine-tune the tensor analysis to capture multiple levels of potentially nested clusters. 
% Tackling this challenge will require us to identify a systematic way to apply tensor decomposition, consider appropriate thresholds (the level of sensitivity)  and a terminating condition. 
%In addition, we want to understand for what datasets and for what related “queries” on this data  would such an approach be most beneficial. 
%This problem is relevant to many different applications of tensor decomposition. To ground our work, we focus our work on online forums, which is an interesting case study for the aforementioned problem. 
In the absence of proper ground truth, we evaluate our approach with synthetic data and test 
its sensitivity to different parameters.
% As a lack of proper ground truth, we provide the proof of the effectiveness by applying \algo on synthetic tensors with both hierarchical and non-hierarchical multi-dimensional clusters injected in it. 
We also apply \algo on five real datasets which involve the activities of users in online discussion platforms, such as security forums. 
This analysis helps us reveal clusters of users with interesting behaviors, including but not limited to early detection of some real events like ransomware outbreaks, the emergence of a black-market of decryption tools, and romance scamming. To maximize the usefulness of our approach, we develop a tool which can help the data analysts and overall research community by identifying hierarchical structures. \algo is an unsupervised approach which can be used to take the pulse of the large multi-modal data and let the data discover its own hidden structures by itself.  

\end{abstract}

==> arxiv-RECTEN (2)/002-Intro.tex <==
\section{Introduction}
%\vp{A quick stylistic comment: Many of the figures are not following their aspect ratio (because in the code the width and length are violating that ratio), it would be better to avoid defining both height and width, usually it is best to definining the width of the figure as a proportion of textwidth (which is a variable in latex) }

%\risul{thanks professor. trying to fix this}

%\reminder{From V: I think this is not the right format for WWW, looks like the AAAI format not the ACM format}

%\miii{In title: What is "Low Rank" meaning as opposed to high rank? Not sure what is multi-modal either? Do you have something in mind, can you define in intro? I understand multi-dimensional. Modal I don't know what it means, but it could be different.}
%\risul{We have defined modes in approach. Low rank means rank 1}


{\em How can we identify hierarchical clusters in multi-modal data?} To answer this question, we leverage a well-established strategy, tensor decomposition. Tensor itself is a multi-dimensional representation of the data. Here, we call each dimension a ``mode". For instance, any tensor that captures the interaction of users with different threads at different times is a ``3-mode tensor" where the modes are the users, threads, and discretized times. Here, we use the terms {\it multi-modal} and {\it multi-aspect} interchangeably.   

% Tensor decomposition and their applications in mining multi-aspect datasets are ubiquitous and ever increasing in popularity. 

%\miii{Intro to tensors}
Tensor decomposition has emerged as a  powerful
analytical tool with a rich variety of applications, but so far,
focuses more on identifying latent clusters and less on identifying hierarchical structure hiding in the data.
Current tensor-based approaches do an excellent job of identifying with hidden and inherent patterns in the form of clusters.
%\miii{maybe add some examples}
We argue that often behaviors and phenomena have an inherent hierarchical structure, which currently may be missed.
% However, there exist research challenges in the field of data mining that
% need to be addressed, in order for tensor decompositions to claim their position as a de-facto tool for practitioners in pattern discovery.




{\bf Problem:}
The main focus of this work is a relatively less explored question: 
how can we extend tensor decomposition to identify hierarchies
if such hierarchies exist in the data?
The problem we address here is as follows.
We are given a multi-dimensional dataset,  and we seek to  identify the potentially hierarchical structure present in the data. 
%usually without any sort of ground truth,
% It is crucial, therefore, to know whether a
% pattern that we extract actually models the data at hand, or whether it is merely modelling noise in the data. Especially in the age of Big Data, it is imperative to have a quality clustering algorithm which avoids
% interpreting noisy and random variation that always exists in the data.
The key challenge here is that: (a) we do not know a priori anything about the data, such as the number of clusters or levels,
(b) we want to adapt to different levels of "sensitivity"
meaning that different parts of the data may hide more
layers of hierarchy than others.
Understanding the hidden structures, especially hierarchical structures, in the data is always a challenging task. 
We want to build on the power of Tensor decomposition by expanding it to address the above challenges. 
% helps us unveil these structures. However, there have been some shortcomings of the traditional non-hierarchical approach: (i) clusters produced from factorization may consists of several sub-clusters, (ii) it does not provide fine-tuned clusters to dive deep into the root structures. 


\begin{figure}[t]
    \centering
    \includegraphics[width=8.5cm, height=5.75cm]{fig/overview4.png}
    \caption{Output from \algo after applying it on ``Hack This Site" security forum data. Hierarchy up to three levels is presented here.}%\reminder{From V: It may be a good idea for this figure to show the best result or a combo of the system and the best result.}
    \label{fig:ourapproach}
\end{figure}

% Some of the users try to keep these forums really live by initiating a discussion or by commenting in discussion while some may try to exploit this opportunity to form a \textit{Hacker Group} or be an active \textit{Hacker}. Also sometimes users talk about such problems like Ransomware that may outburst in the near future. 
% Our main goal is to catch these types of important events, threads, and users that may catch sight for a security investigator.  


Formally, we state the problem as follows:

\begin{shaded*}
    Given a Tensor $T$, how can we expand the decomposition of $T$ in a recursive manner into a hierarchy of clusters, $C_i$? The input is a tensor and the output is a hierarchy of clusters. 
\end{shaded*}

The problem poses two main challenges:
(a) we want to recursively decompose clusters in each layer of the hierarchy, and (b) we want to identify the right conditions for terminating this process.

% That means, we opt to expand the typical tensor decomposition algorithm recursively to provide clusters in level-by-level manner so that it reveals more fine-tuned and hidden sub-structures.  




{\bf Related work:} 
Despite the vast literature on tensor decomposition, we are not aware of
any work that fully explores the possibility of hierarchical tensor decomposition.
% GROUP work in families:
We can group prior efforts into three main categories:
(a) discovering hierarchical structures using non-tensor approach,
(b) recursive hierarchical use of tensor decomposition \cite{abdali2020hijod, wang2015towards},
%\miii{has there been any such work??? Maybe say "hierarchical decomposition without using tensors?}
and
(c) other tensor decomposition approaches and applications.
%analysis with a focus on “carefully” tailoring granularity,
We discuss these efforts in detail in  the {\em Related Work} Section.
%~\ref{sec:related}.

%However, current works focus on solely identifying ‘Hackers’. 


{\bf Contribution:}
% Our proposed method, \algo, offers a systematic hierarchical approach to delve deeper into the multi-modal data to unravel the hidden structures leveraging the traditional tensor decomposition method. 
As our key contribution, we propose \algo, a  hierarchical soft clustering
%\miii{Is it soft coclustering? yes} 
approach based on tensor decomposition. 
Our approach provides the required mechanisms for recursively decomposing clusters, and  for terminating this recursive process. 
% Our key contributions are:
% (a) {\bf Algorithm.} We propose, \algo, a systematic and novel unsupervised algorithm to expand tensor decomposition recursively in hierarchical manner and reveal hidden patterns from the input Tensor in much more efficient and hierarchically structured fashion, and
We  evaluate our proposed algorithm using both synthetic and real data.
We use the  synthetic data in order to evaluate the performance in the absence of proper ground truth. control the underlying structure of the dataset.  We also use this synthetic data to evaluate the sensitivity of three internal parameters, which enables us to provide recommendations for hands-free operation. In our evaluation, we find that \algo performs favorably when compared to other traditional and state-of-the-art methods. 


We provide indirect evidence of the usefulness of \algo in isolating the data patterns by finding interesting clusters. These clusters correspond to online users with interesting behaviors.
We conduct a large scale study on 5 real datasets using \algo and explore the hidden hierarchical patterns within these datasets. 
For example, we analyze
three security forums: Offensive Community \textbf{(OC)}, Ethical Hacker \textbf{(EH)}, Hack This Site \textbf{(HTS)}. 
%from 2013 to 2017 as shown in Table~\ref{tab:stat}. 
We also apply \algo on two other datasets: a MultiPlayer Game and Hacking Cheats ({\bf MPGH}) forum dataset, and a dataset of authors on GitHub. We identify interesting activities there as well including revenge hacking, romance scamming, and ransomware explosion as we discuss later in {\em Application Results and Observations} Section.







{\bf A usable platform.} As a tangible contribution, we develop a powerful user-friendly platform that will be useful to researchers, security analysts, and data specialists. The key advantages of \algo platform are as follows:
(a) it operates in an unsupervised way, 
%though the user has the ability to \enquote{interfere} if they opt do so,
(b) it is user-friendly by being 
both automatic  and customizable, and 
(c) it provides an interactive way of getting clusters in a hierarchical manner which helps to understand the inherent patter in the original input tensor.

% and the dynamics of the related authors, threads, and times of interest. 

%\algo can bring in enormous benefit for the research communities, security analysts, and cyber-security related law enforcement authorities which actually motivated us to deploy \algo tool as an addition to software industry, discussed later in Section \ref{sec:vision}.




%\algo extracts a total of 52 clusters from these forums. 

% which consists of three forums: Offensive Community \cite{oc}, Ethical Hacker \cite{ehacker}, Hack This Site! \cite{hthissite},  although we only show results from the Offensive Community forum here.
% Due to space limitations we focus on the Offensive Community forum that span 5 years and contain 5412 users, 23918 posts and 3214 threads.
%\miii{Not sure if we need this: We identify 25 clusters with our tensor-based clustering, whose sizes range from X to Y users and Y to W threads.}
%We highlight some key and indicative results below.

%pecifically, we find  clusters, which fall in the following categories: (a) {\bf 26\% of the clusters correspond to real security events}, such as attacks, (b) {\bf 22\% of them represent black market communities} for malware tools and services, and (c) {\bf 32\% of them represent security tutorials, events and communities}, with most tutorials sharing malware and penetration techniques. We highlight nine  clusters in  Table~\ref{tab:1result} and list some indicative clusters below.
%\miii{Low priority: Maybe not focus only on OC if we can add other exciting results, but this is ok as well?}

%\miii{Let's mention "specific" results}


%,  27 threads, 43 users in 20 different times useful and worth investigation



 %{\bf a. Clusters of hacking services activity:} An indicative cluster  (31 users, 125 threads in OC) captures an underground market activity with 34 sellers and buyers, who exchange, buy/sell and talk about hacking services. In our investigation step, we find that a key activity is a discussion and deals around ransomware, and  specifically SimpleLocker, in Dec 2015 and again in Feb 2016. This mirrors the emergence of SimpleLocker, which gained prominence in Dec of 2015.

 %{\bf b. Clusters of malicious announcements:} A cluster  in this category (42 users, 65 threads in OC) revolves around announcing hacking events and related discussions, including bragging.  The cluster exhibits a surge of activity, when user V4ND4L claims to have hacked into Facebook. Furthermore, the cluster includes an invitation by the same user to form a group to hack into a bank!

 %{\bf c. Clusters of malicious tutorials:} A cluster here (55 users, 120 threads in OC) revolves around tutorials on how to break into systems and spread viruses effectively. Our approach identifies the most active users,  Dragunman and Pratham, who are sharing information on hacking into banks, and hacking into WiFi/mobile credentials respectively.


%{\bf Going beyond security forums.} Although we focus primarily on security forums in this paper, \algo can be used on other types of forums. As a proof of concept, we applied our approach on an online gaming forum, MultiPlayer Game and Hacking Cheats (MPGH), and found interesting  activities there as well,  including revenge hacking and romance scamming, as we discuss later.


%~\ref{sec:vision}.

%\miii{Not sure what to keep from below}



% Our approach forms an important first step in quickly processing a forum in the search of large events of interest
% in an unsupervised learning fashion.




==> arxiv-RECTEN (2)/003-Data.tex <==
\section{Datasets}
\label{sec:data}

To show the effectiveness of \algo, we apply it on a total of five datasets from our archive. The datasets include (i) three security forum datasets, (ii) one gaming forum dataset, and (iii) malware repositories and their authors from GitHub dataset. All these datasets are private except the gaming forum and we wish to make these public once the work is accepted.  We provide a brief description of these datasets below.

{\bf a. Security forum datasets. }
We utilize the data that we collect from three security forums: Offensive Community (OC), Hack This Site (HTS), and Ethical Hackers (EH) ~\cite{secforums}. All the forums are in English language. In these forums,
{\it users} initiate discussion {\it threads} 
in which other interested users can {\it post} to share their opinion. The discussions expand both ``white-hat" and ``black-hat" skills. The datasets of the security forums span 5 years from 2013 to 2017.
Each tuple in each of our datasets contains the following information: user ID, thread ID, post ID, time, and post content. 

{\bf b. Gaming forum dataset. }
We also apply \algo on another different type of online forum of larger size to see if our approach would work equally well. For this reason, we apply our method on an online gaming forum, Multi-Player Game Hacking Cheats (MPGH) \cite{secforums}. MPGH forum is one of the largest online gaming communities with millions of discussions regarding different insider tricks, cheats, strategy, and group formation for different online games. The dataset was collected for 2018 and contains 100K comments of 37K users~\cite{pastrana2018crimebb}. The format of each tuple is the same as security forum datasets. 

\begin{table}[t]
    \caption{Basic statistics of our datasets.}
    \footnotesize
    \centering
    \begin{tabular}{|P{0.27\linewidth}|P{0.08\linewidth}|P{0.20\linewidth}|P{0.1\linewidth}|P{0.09\linewidth}|}
         \hline
         \textbf{Dataset} & \textbf{Users} & \textbf{Threads/ Repositories} &  \textbf{Posts} & \textbf{Active Days}\\
         \hline
         Offensive Comm. & 5412 & 3214 & 23918 & 1239\\
         \hline
         Ethical Hacker &  5482 & 3290 & 22434 & 1175\\
         \hline
         Hack This Site & 2970 & 2740 & 20116 & 982 \\
         \hline
         MPGH & 37001 & 49343 & 100000 & 289 \\
         \hline
         GitHub & 7389 & 8644 & - & 2225 \\
         \hline
    \end{tabular}
    \label{tab:stat}
    \vspace{-4mm}
\end{table}


{\bf b. GitHub dataset. } GitHub platform 
enables the software developers to create software repositories in order to  store, share, and collaborate on projects and provides many social-network-type functions.
%and benefit from version control.

We  define some basic terminology here. 
We use the term {\it author} to describe a GitHub user who has created at least one repository.
A {\it malware repository} contains  malicious software and
% \ri{A {\it user} is the one having an account in \github whereas an {\it author} is the user having at least one repository.}
%In our context, {\em malware author} 
a {\it malware author} owns at least one such repository.
Apart from creating a repository, users of GitHub 
%\ri{Would it be good to differentiate between user and author as one reviewer objected he got confused}
can perform different {\it types of actions} including {\it forking, commenting}, and {\it contributing} to other repositories. {\it Forking} means creating a clone of another repository. A forked repository is sometimes merged back with the original parent repository, and we call this a {\it contribution}. Users can also {\it comment} by providing suggestions and feedback to other authors' repositories. Each tuple is represented in the format: malware author ID, malware repository ID, action type, time, and repository content.  


% Our peliminary work, SourceFinder \cite{rokon2020source}, found a surprising number of malware repositories because of the lack of strong check from \github.
%\ri{Is "lack of strong check" seeming out of nowhere? why check?}
We use a dataset of 7389 malware authors 
and their related 8644 malware repositories, which were identified by prior work~\cite{rokon2020source}.
This is arguably the largest malware archive of its kind with repositories spanning roughly 11 years.

The basic statistics of the datasets are shown in Table \ref{tab:stat}.



==> arxiv-RECTEN (2)/0040-approach.tex <==
\section{Our Approach}
\label{sec:approach}


We present, \algo,  a novel tensor-based multi-step recursive approach that identifies patterns in an unsupervised way.  
Fig. \ref{fig:ourapproach} provides
the basic workflow of \algo. Algorithm 1 also provides the high level pseudo-code. The simplest idea is that: we decompose a tensor into clusters at level 1. Each cluster at level 1 will be considered as another tensor to be decomposed into clusters at level 2 and so on until some stopping criteria are met. We present the overview of  \algo in three steps: a)  Tensor-based clustering, b)  Prepare for the next level decomposition, and c) Termination conditions. We now discuss the basics of tensor decomposition and then the algorithmic steps below.


%\miii{Low: Do we use these metrics below? If not, we can defer and define all metrics in one place.}


{\bf Tensors and decomposition.} A d-mode tensor~\cite{kolda2009tensor} is a d-way array (here $d\geq3$). So, we call \scalebox{0.85}{$I \times J \times K$} tensor a  ``3-mode'' tensor where ``modes'' are the number of dimensions to index the tensor; the ``modes'' can be $A={\{a_1, a_2, ..., a_I\}}, B={\{b_1, b_2, ..., b_J\}}$, and $C={\{c_1, c_2, ..., c_K\}}$. Each 3D {\it element/entity} of the tensor, \textit{X(i,j,k)}, captures the interaction of  $a_i$, $b_j$, and $c_k$ or zero in the absence of any interaction. 
In a decomposition, we  decompose a tensor into \textit{R} rank-one components, where \textit{R} is the rank of the tensor, as shown in Fig.~\ref{fig:2tensor}. That means, tensor is factorized into a sum of rank-one tensors i.e. a sum of outer products of three vectors (for three modes):  \scalebox{0.85}{$X \approx \sum_{r=1}^{r=R} A(:,r)\circ B(:,r)	\circ C(:,r)$} where \scalebox{0.85}{$A \in R^{I \times R}$ , $B \in R^{J \times R}$, $C \in R^{k \times R}$} and the outer product is derived by \scalebox{0.85}{$(A(:,r)	\circ B(:,r)$ $\circ C(:,r))(i,j,k)$ = $A(i,r)B(j,r)C(k,r)$} for all \textit{i, j, k}.
 %\vp{make sure you are consistent with the notation e.g., X[i,j,k] vs. U(:,r)} 
Each component represents a latent pattern in the data, and we refer to it as a {\bf cluster}.
For example, one such cluster in OC security forum  represents a group of 29 users that are active in the first weekends of July 2016 and discuss ``multi-factor authentication failure" in a group of 72 threads.
%\miii{Do we have a real *intuitive* example we can use here?}
Each cluster is defined by three vectors, one for each dimension, which show the ``{\it Participation Strength}" of each element for that cluster.
Typically, one considers a threshold to filter out elements that do not exhibit significant {\it Participation Strength}, as we discuss later.





\subsection{Step 1: Tensor-based clustering} 

%\rismi{ This whole step 1: I shrunk to three "questions"-- Risul+Vagelis please review}


We provide a quick overview of the challenges  and algorithmic choices in our approach. 

\textit{a. What is the ideal number of components to target in the decomposition?} To answer this question, we use the AutoTen method~\cite{papalexakis2016automatic} and find the rank (R) of the tensor, which points to the ideal number of clusters to be decomposed into. AutoTen uses the {\it Core Consistency Diagnostic} metric in {\fontfamily{qcr}\selectfont CP\_ALS} and {\fontfamily{qcr}\selectfont CP\_APR} to find two probable ranks and finally chooses the max rank for the decomposition. So, the final rank, $R$, of a tensor is computed as follows: $R = max(R_{{\text{\fontfamily{qcr}\selectfont CP\_ALS}}}, R_{{\text{\fontfamily{qcr}\selectfont CP\_APR}}})$.

\textit{b. How can we decompose the tensor?}  We use the non-negative Canonical Polyadic or CANDECOMP/ PARAFAC (CP) decomposition to find the clusters.
%\cite{faber2003recent} 
%\cite{faber2003recent} \vp{this is an awkward citation for PARAFAC. Maybe cite Kolda's survey paper or something instead} 
%The factorization may contain negative numbers in the decomposed components whereas our strategy of capturing the interaction between users and threads at different times is inherently non-negative.  
\algo achieves this non-negative factorization by adding the non-negative constraint in CP decomposition.
%\cite{shashua2005non}. 
%\vp{I would say let's cite something for the non-negativity constraint here too, because it appears that it's not been done before.}


\textit{c. How can we strike a balance on cluster size?}
Each cluster, derived from a 3D tensor, is defined by three vectors whose lengths are equal to the dimensions of the tensor as shown in Fig.~\ref{fig:2tensor}. However, \algo provides the functionality of having clusters with significant elements only. Therefore, we need a threshold to determine \enquote{significant participation in the cluster}, which is a common practice for (a) avoiding unreasonably dense clusters~\cite{sapienza2018non}, (b) enhancing interpretability, and (c) suppressing noise.
So, the challenge is to impose this sparsity constraint and eliminate the need for ad-hoc thresholding to find the clusters with only significant entities. 
% So, we need to address the  question: \textit{How can we impose this sparsity constraint and eliminate the need for ad-hoc thresholding to find the clusters with only significant users, threads and times?} 
Our solution is to add $L_1$ norm regularization with non-negative CP decomposition. $L_1$ regularization pushes the small non-zero values towards zero.
%\cite{neumaier1998solving}. 
Therefore, for each vector, we filter out the zero-valued elements and produce clusters with significant elements only. In this way, we can eliminate the noisy entities having the least significant contributions in the cluster. The final model that we use for finding the clusters looks like this:

\scalebox{0.70}{%
$ \underset{A\geq 0, B\geq 0, C\geq 0}{\text{min}} \left\lVert X-D \right\rVert_{F}^{2} + \lambda ( \sum_{i,r} |A(i,r)| + \sum_{j,r} |B(j,r)| + \sum_{k,r} |C(k,r)|) $
}
where $\lambda$ is the sparsity regularizer penalty (set to 1) and \scalebox{0.75}{$D = \sum_{r} A(:,r)\circ B(:,r)\circ C(:,r)$}. To find the clusters, we solve the above equation. Since the equation is highly non-convex in nature, we use the well-established Alternating Least Squares (ALS) optimizer as the solver.  
An example of a cluster after filtering is shown in Fig.~\ref{fig:cluster_example}.
%~\ref{sec:results}.

%\miii{How is the average defined? For that vector? can you cite previous work for doing this}. 


\begin{figure}[t]
    \centering
    \includegraphics[ width=\linewidth]{fig/tensordiagram.png}
    \caption{Visualization of tensor decomposition.}
    \label{fig:2tensor}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[ width=\linewidth, height=5.5cm]{fig/example_cluster.png}
    \caption{An example of a cluster (28 Users, 70 Threads, 6 Weeks) from OC. The intensity in each vector helps us identify users, threads and time intervals that are ``important" for the cluster. }
    \label{fig:cluster_example}
    
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[height=5.5cm, width=\linewidth]{fig/example_cluster.png}
%         \caption{An example of a cluster (28 Users, 70 Threads, 6 Weeks) from OC. The intensity in each vector helps us identify users, threads and time intervals that are ``important" for the cluster. }
%     \label{fig:4cluster_example}
% \end{figure}




\subsection{Step 2: Processing for the next level decomposition}
\label{subsec:next_level_prep}
Having obtained the clusters at level 1 (in general at level $l$), our next goal is to decompose each cluster into further clusters if termination conditions are not met. 
%In future, we refer to a cluster, ready to be decomposed for the next level,  as ``tensor". 
The intuitive idea is to introduce some disturbance in the cluster so that the hidden patterns further gets isolated in separate clusters at the next level. That means, if there are multiple hidden structures/patterns are convoluted in a particular cluster, we enforce the cluster to be divided into further clusters. To achieve this goal, we face the following algorithmic challenges: 

{\bf Rank modification. } 
The main mathematical challenge in this phase is to answer the question: ``{\it How can we get the clusters ready to be decomposed further for the next level?" }  because the rank of every cluster is 1. That is why these clusters can not be decomposed directly. To decompose a cluster at level $l$ into multiple clusters we need to have the rank of the cluster at level $l$ greater than one. We propose to achieve this by introducing some disturbance in the cluster at level $l$. Recall that a cluster is also a tensor of rank one. Therefore, we  propose to introduce some disturbance by zeroing-out some carefully chosen subset of entities from this rank one tensor and make it ready to be factorized into further clusters because this zeroing-out strategy changes the rank of the cluster to $\geq 1$.


{\bf Choosing the ``target entities'' to zero-out.} The next question inherently comes into the picture is that ``{\it Which entities to choose for zeroing out? }". To zero out, we propose to select the non-zero valued entities stochastically but biased towards their values in the cluster. 

Let's assume 
%$N$ be the set of non-zero entities and $Z$ be the zero-valued entities in 
$C_l$ be the rank-one cluster  at level $l$, $l \geq 1$. We get the processed Tensor $T_l$ with rank, $r>=1$, in the following manner:

%$$T_l = C_l . / B $$

%where $./$ is the Hadamard Product and B is the Basis Tensor for Hadamard Product. This element wise Hadamand Product between $C_l$ and $B$ zero-outs some entities from $C_l$ and makes it prepare for the next level decomposition, ($r>=1$).   To calculate the Basis Tensor, $B$, we first take an all-ones tensor with dimension $I \times J \times K$.
We choose a subset of elements/entities stochastically biased towards their values, $C_l(i,j,k)$, and replace those with 0. We propose that the probability of an entity getting chosen to be replaced with 0 is inversely proportional to $C_l(i,j,k)$. That means, the higher the entity value, $C_l(i,j,k)$, the lower the probability of getting replaced with 0. Therefore, the probability of getting chosen for any non-zero point $p$ at $(i,j,k)$ for 3-mode Tensor, is formulated by the following formula:
$$P(\text{p is chosen}) = \frac{\frac{1}{C_l(p)}}{\sum_{q\in C_l} \frac{1}{C_l(q)}}$$  where $C_l(p) = C_l(i,j,k)$. After replacing the chosen entities with zero, we get the processed tensor, $T_l$, ready to be decomposed for the next level, $l+1$. In summary, we zero out some values from $C_l$ and get it ready for the next level decomposition.


{\bf Amount of deletion. } The next question arises is that: ``{\it What amount of entities should be zeroed-out?}" We propose to select $\epsilon\%$ of the total non-zero valued elements in $C_l$. We choose the next integer value after $\epsilon$ if we can not have exactly $\epsilon$. We find the suitable value of $\epsilon$ empirically described in {\it Evaluation of \algo} Section.


\subsection{Step 3: Termination condition}
\label{subsec:termination_condition}
We stop the recursive procedure of clustering when one of the two termination conditions is met:

{\bf a. Termination condition 1: Tensor size significantly small. } This preliminary termination condition suggests that when the cluster/tensor size is significantly small, we can not further break it. Now the obvious question is: ``{\it When do we call a cluster ``significantly small"?}" We say a cluster significantly small when the number of non-zero values in it
%largest mode (mode with highest dimension) 
becomes less than {\it k\%} of the average number of non-zero values in the sibling clusters at that level. Let's say, at level $l$, tensor $T_{l-1}$ is factorized into a set of clusters $Y_l$, $x \in Y_l$ be a member cluster whose recursive factorization decision we are going to take,  $Z_l = Y_l \setminus x$ is the set of sibling clusters of $x$, $n(c)$ is the number of non-zero elements in cluster $c$, and $N(Z_L) = \frac{\sum_{z\in Z_l} n(z)}{|Z_L|} $ is the average number of non-zero elements in the sibling clusters, $Z_L$. Therefore, according to termination condition 1, we will not factorize cluster $x \in Y_l$ if:

 $$\frac{n(x) * 100 }{N(Z_l)} < k $$
 
%\ref{} suggests that tensor yields very small clusters when factorized into number of cluster s more than the actual rank. 



{\bf b. Termination condition 2: AutoTen rank=1. }
Another termination condition of the recursive factorization  is that after preparing the cluster for the next level factorization, \algo will not factorize that particular cluster if its ideal rank provided by AutoTen is still 1. To summarize, if $R == 1$ for the cluster after processing, we skip the factorization of that particular cluster.


\begin{shaded*}
{\it Claim 1. Using \algo, zeroing-out of subset of non-zero entities from the rank-1 tensor changes the rank to $\geq 1$.} 
\end{shaded*}

We present the intuition behind proving this claim here. Lets say, we have a tensor $T$ and after deletion of some non-zero elements, we have the new tensor $\dot{T}$. Basically, we have to prove $rank(\dot{T}) - rank(T)>=0)$ given the situation.

Assume that, in \algo, zeroing-out of some non-zero entities in the rank 1 tensor leads to rank zero. But from the definition of rank-zero tensor, we know that rank-zero tensor has only the zero-valued elements, and thus introduces contradiction because it is not possible to have a zero-tensor in \algo. So, zeroing out can never lead to rank zero tensor, i.e. $rank(\dot{T}) - rank(T) \nless 0)$. 

Now, during zeroing out in \algo, we actually get a new tensor, $\dot{T}$, by zeroing-out non-trivial non-zero entries from $T$. Mathematically, this is done using element-wise Hadamard Product between the rank-one tensor, $T$, and a basis tensor $B$ i.e. $\dot{T} = T ./ B$ where $B$ is the basis tensor with elements either set (1) or reset (0). 
This type of zeroing-out is equivalent to introducing at least zero perturbation. Therefore, we can say $rank(\dot{T}) - rank(T)>=0$.


\begin{algorithm}[t]
\DontPrintSemicolon
  
  \KwInput{Root Tensor, T} %\tcp*{this is a comment}
  \KwOutput{Clusters arranged in hierarchical tree format}
  %\KwData{Testing set $x$}
  %$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
  Clusters = [clusters from first level Decomposition of given root tensor, T]\\
  Final\_clusters\_tree.insert(T,null)\\
  Final\_clusters\_tree.insert(Clusters,T)\\
  \While{ Clusters != empty}
  {
        Temp\_clusters=[]\\
        \For{ each C in Clusters}
        {
            \If{Termination Condition 1}
            {
                continue
            }
            %Calculate Basis Tensor B\\
            Construct $C_{new}$ by removing some entities from $C$ \\
            \If{Termination Condition 2}
            {
                continue
            }
            Decompose $C_{new}$ into new clusters $C_i$'s\\
            Temp\_clusters.insert($C_i$'s)\\
            Final\_clusters\_tree.insert($C_i$'s, C)\\
        }
        Clusters=Temp\_clusters\\
  }
    \Return Final\_clusters\_tree\\

     



\caption{
\begin{shaded*}
{\bf RenTen({\it T})} Algorithm to factorize a Tensor recursively to have hierarchical clusters.
\end{shaded*}
}


\label{algo:recten}
\end{algorithm}















\begin{comment}




\textbf{Step 2.1. Content-Based Profiling:} We propose to profile clusters using content with the aid of two interconnected steps.

{\bf a. Cluster characterization:}
We identify the top {\it N}  keywords using TF-IDF from the first post of each thread in each cluster. Prior work recommends the use of the first post of a thread for capturing the focus of a thread~\cite{Joobin}. We use the term {\bf cluster keywords} to refer to this set of words. These keywords can already provide a feel for the nature of the cluster,
but we also use more sophisticated techniques in the next step.


\textbf{b. Cluster labeling:} We give the end-user the ability to define classes of interest that we then use to label the clusters. 
For ease of use, the user can define a class by providing 
 a bag of words. To label the clusters,
 we compare these bags of words with the cluster keywords from the previous step.

To demonstrate this capability, 
 we start with a group of classes that would be of interest to a security analyst.
 Specifically, we adopt the following classes of interest from  prior work~\cite{Joobin},
 which defines four types of threads:
{\bf Announcement type (A)}  where people announce news and events, including  hacking achievements and cyber-attacks; {\bf Product type (P)},  where people buy or sell hacking services and tools; {\bf Tutorial type (T),}  where users post tutorial on how to secure or hack into systems;  and,  {\bf General Discussion type (G)}, which is the category for all threads not in the above categories. 
%~\cite{Joobin}

We then  calculate how ``relevant" each cluster is to each class type. 
For consistency, we have adopted the 
same definitions
%same {\it N}  keywords  to define
for these categories as the aforementioned work.
To do this,
we compute the Jaccard Similarity~\cite{choi2010survey} between the \textit{cluster keywords} and the keywords that define each class type. We  label the cluster as \textit{A, T, P, G} type based on the highest Jaccard Similarity score. A cluster can be labeled as \textbf{Mix} type, if the similarity scores of different types is within a close range 
(defined as \pm 0.02). 
%\miii{Explain what is the criterion for Mix vs pure cluster? We don't need major details, but even something quick: when similarity for more than one cluster is above .... then we consider it a Mix. Or We consider a pure cluster only when Similarity score is higher by X compared to second highest...}


% For example, if the similarity score between {\em cluster keyword}  and {\em A} type keyword is the highest, we label the cluster as Announcement type cluster and so on. Note that a cluster can be labeled as a mixture of \textit{A, T,} and \textit{P} types. 


%{\bf Step 2.2: Understanding the clusters:} 
{\bf Step 2.2. Behavior profiling:} 
To provide more information per cluster,
we  use behavioral properties, which capture how users and threads interact with each other over time.
This gives rise to metrics such as, number of users per cluster, number of threads per cluster, duration of a cluster (defined as the difference between the last and the first post of the cluster) etc. We provide the following groups of capabilities and plots to the end-user:

\textbf{a.} \textbf{Basic Distribution plots} of metrics of the clusters in a forum, such as the distribution of \#users, \#threads, \#active days etc. per cluster of the forum.

\textbf{b.} \textbf{Scree-plots} of metrics of clusters, which capture the pair-wise relationships of different metrics of clusters, 
such as \#Threads vs \#Users for each cluster of the forum as shown in Fig.~\ref{fig:screeuserthread} and \ref{fig:screedurationactivedays}. %\miii{check if this is the correct figure}

\textbf{c.} \textbf{Heat map visualizations} of the clusters and the relative strength of their behavioral metrics.
Currently, we use ten behavioral metrics that include
the average (over the cluster): average post length per user, number of threads initiated per user, comment to thread participation ratio of the users,
number of comments per user, number of active days of the threads etc.
We normalize the values of the averaged  metrics and present the behavioral profiles  using a heat-map-style plot 
 as we show, and discuss later, in Fig.~\ref{fig:5profile_cluster}.
 
The visual depiction helps an analyst to quickly gauge the behavioral profile of the clusters and spot differences. Also we expand this functionality by developing an automated capability to report the anomalous cluster/s using standard DBScan anomaly detection algorithm \cite{sheridan2020application} in these profiles. We discuss this finding in ``Result'' Section. 
%\ref{sec:results}.


%\miii{It would be more complete to refer to all metrics, or at least metrics that we may end up using later we we discuss this plot}

%\miii{==== BEGIN The below needs to most likely go ====}




%\miii{==== END The above needs to most likely go ====}

\begin{figure*}[t]
\begin{multicols}{4}
    \includegraphics[width=\linewidth,height=4cm]{fig/user_cluster.png}\par a)
    \includegraphics[width=\linewidth,height=4cm]{fig/thread_cluster.png}\par b)
    %\includegraphics[width=\linewidth,height=4cm]{fig/duration_cluster.png}\par c)
    \includegraphics[width=\linewidth,height=4cm]{fig/activedays_cluster.png}\par c)
    \includegraphics[width=\linewidth,height=4cm]{fig/engagement_cluster.png}\par d)
\end{multicols}
\caption{Sorted a) \# of user b) \# of threads c) Active days d) Average \# of Engagement by users in A, T P, Mix/G type clusters in OC, EH and HTS forums.}
\label{fig:clusterproperties}
\end{figure*}


\begin{figure*}[t]
\begin{multicols}{4}
    \includegraphics[width=\linewidth,height=4cm]{fig/scree_user_thread.png}\par a)
    \includegraphics[width=\linewidth,height=4cm]{fig/scree_duration_thread.png}\par b)
    %\includegraphics[width=\linewidth,height=4cm]{fig/scree_duration_activedays.png}\par c)
    \includegraphics[width=\linewidth,height=4cm]{fig/scree_duration_percentageactivedays.png}\par c)
    \includegraphics[width=\linewidth,height=4cm]{fig/scree_thread_engagement.png}\par d)
\end{multicols}
\caption{Scree plots of a) \# of user vs \# of threads b) Active Duration vs \# of threads c) Percentage of Active Days vs Active Duration d) Avg \# of Engagement vs \# of threads in A, T, P, Mix/G type clusters of OC, EH and HTS forums. [Active Duration is the difference between the posting time of the first and last post in a cluster.]}
\label{fig:scree}
\end{figure*}



%\vp{is this explained somewhere in detail?}
%\miii{Are we profiling per user or in general behavior, avg number of new threads per active day etc}. 

%\miii{I think this should be here, no?}

%\miii{Figures need caption that describe the figure properly: Typically one wants to explain the x and y axis, give context as to the data described, and if possible a key message "The top highest spikes correspond to xxxx}

\subsection{Step 3: Investigation of clusters}  


We develop a suit of capabilities that can help automate
an  in-depth investigation of the clusters coming from the previous steps.
% The goal of this step is to provide a more in-depth investigation for the clusters we have identified and profiled in the previous step.
% Given clusters and their profiles shown, we can go deeper and explore the dynamics within the cluster. 
Although this can be done manually, the goal is to
make the life of an analyst easier. 
Our platform provides the user with well-organized and easily accessible information trying to strike the balance between
being informative and intuitively interpretable.
% in a way that can facilitate the analysis of a forum and its identified clusters.
% For example, Table~\ref{tab:clustsummary} provides a bird's-eye view of the clustering decomposition and the relative sizes.
Moreover, we develop two ways that the end-user can summarize the clusters: (i) \storyline, and (ii) \tableview. 



{\bf Step 3.1. Creating the \storyline:} We develop a systematic and, arguably, more interpretable method to 
capture the essence of a cluster by highlighting the {\it k} most indicative  threads in 
a non-decreasing temporal order as shown  in Fig.~\ref{fig:event_report}. To accomplish this effectively, we follow the process described below.


% \risul{
% First, for each cluster, we create the document corpus considering the \textit{title} of each thread as ``document'' to train a LDA Bag-of-Words model \cite{sharma2017survey}. Then we extract the topics from the corpus where number of topics is equal to the number of threads in the cluster and number of words in each topic is equal to the average number of  words in the titles after standard preprocessing. Note that a topic is represented as a weighted list of words. Then we calculate the \% of topics a document is about (\textit{topic scores} for each document) and from there we assign each document a topic depending on the highest \textit{topic score}. In the next phase, we find the distribution of the number of documents per topic and choose the most representative topics,\textit{(dominant topics)}, from there. Note that, from each cluster, we only chose the minimum sized {\it dominant topics} set which represent at least 70\% of the ``document''. Now, for each of the \textit{dominant topics}, we find the top {\it k} [default=3] documents({\it titles}) having highest \textit{topic scores}, discussed earlier, in a story-line (non-decreasing timeline) manner demonstrated in Fig. \ref{fig:event_report}. Just by gauging through the \storyline, the end-user can have a complete feel of the discussion going on in a cluster. 
% }

Identifying the important threads for the cluster is calculated in the following stages.
In stage one, we find an extended list of topics, $T_{ext}$, for the whole cluster. To do this, we use the commonly-used LDA Bag-of-Words model \cite{sharma2017survey}, and  we focus on the titles of the threads in the cluster. 
%%%% ---- Detail ***** future *****
In stage two,  we calculate the {\it relevance scores} $R(t)$ of each thread with respect to each topic $t \in T_{ext}$. 
%\% of topics a thread is about,(\textit{topic scores}), and 
We associate each thread with the topic with highest {\it relevance score}.
In stage three, we find the most representing topics, $T_{dom}$, of the cluster. To achieve this, we find the distribution of the number of threads per topic and from there we choose the  list of \textit{dominant topics, $T_{dom}$},
which we define as the minimum number 
of topics that represent at least 70\% of the threads.

In stage four,  we identify the top \RelThreads most relevant threads  based on their relevance score for each of the dominant topics $T_{dom}$. We then present them in a non-decreasing temporal order as shown in Fig.~\ref{fig:event_report}. Note that the parameter 
\RelThreads has a default value of 5, but the end-user can adjust it to her liking.

The above process is one of the possible ways to achieve this goal. In the future, we will consider and evaluate alternative approaches. For example, 
here,  we focus on the titles as we want to have the title of thread ``tell the story" in a visceral and intuitive way for the user. In the future, we will consider the text of the whole thread to find topics and consider more involved topic extraction methods.




{\bf Step 3.2. Creating the \tableview:}
We provide an alternative way to view all the clusters 
in the forum in a way that puts emphasis on key authors and key threads. 
 This \tableview can provide compact event summarization and key entities in each cluster.
 %as well as in the whole forum. 
 We argue that this may be appealing
for a different type of analysis.
 Table~\ref{tab:1result} demonstrates the \tableview that we provide.
In our platform, we have clickable links that one can follow to investigate these entities of interest providing an interactive capability. We now present the generation of the columns of Table~\ref{tab:1result}.
 

{\bf a. Identifying important entities: users, threads and time intervals.}
We propose a method to identify the most dominant users, threads, and time periods, where significant activity takes place and populate the columns 4, 5, and 6 in Table~\ref{tab:1result}. Specifically, we propose to identify the top \textit{k} entities from each cluster, where $k \geq 1$ with the default being \textit{k}=3. 
We use the factorized vectors to gauge the ``importance" of an entity in a cluster as shown in Fig.~\ref{fig:4cluster_example}. 
The  black circles show the entities with the highest ``Participation Strength''. From each of the top {\it k} weeks, we also report the most active day in terms of highest \# post made in that week.
% , which are the best candidates for helping us understand the nature of the cluster.
Note that the parameter \textit{k} can be modified by the end-user
to adjust to her preference or type of investigation.




{\bf b. Representing the nature of the cluster in \tableview:}
We present another way to capture the essence of a cluster,
which we provide as text in the last column of Table~\ref{tab:1result}. 
Obviously, there are many ways to achieve this.
%  from the list of the most dominant \textit{cluster keywords} (50 most important words in the cluster) can provide significant information. 
%For example, one  such cluster talks about the outbreak of SimpleLocker, and the term ``SimpleLocker" is the second most frequent keyword in its \textit{Cluster Keywords}.
We opt to report the most dominant topics, $T_{dom}$, per cluster which is a common practice to represent and interpret events~\cite{shi2019human,shi2020event,mehta2019event}.
We have already discussed a method to identify the dominant topics above, which can be provided in the final column in Table~\ref{tab:1result}. However, we can also allow the end-user to modify the text with more expanded notes and explanations by elaborating on the dominant topics. Note that in the table here,  we have manually expanded on the dominant topics and reconstructed the events within each cluster to make it easier for the reader to see what
the cluster is about.




%\miii{maybe we can put a forward reference IF we can find that say the top 20 keywords for SimpleLocker event contain SimpleLocker! :-)}











=========== COmments starts here =============

\textbf{b) Identifying entities of importance in a forum.} 
We propose a way to identify important entities for the forum as a whole by its propensity to participate in clusters. 
We use the term  \textbf{Participation Frequency} of an entity to refer to the  number of clusters in which that entity appears. We identify
and report the top \textit{k} entities depending on their Participation Frequency. For example, user ``V4ND4L" appeares in  7 clusters  (Participation Frequency=7), which suggests s/he may be  an influential person in the OC forum.


============ step 3 =============
\textbf{(a) Identifying entities of importance in a cluster.}
% For ease of presentation, we discuss identifying important threads below, but we use the same approach for users and time intervals. 
We propose to identify the top \textit{k} entities from each cluster, where \textit{k}=[1,3,5,10] with the default being \textit{k}=3. 
We use the tensor decomposition vector to gauge the ``importance" of an entity in a cluster as shown in Fig.~\ref{fig:4cluster_example}. 
The  black circles show the entities with the highest ``Participation Strength'',
which are the best candidates for helping us understand the nature of the cluster. 
% With the same reasoning for users and intervnals,
% we identify the the top \textit{k} entities from each cluster.
%\miii{Not sure what this leads to}. 


{\bf Step 3.2. Combining all previous information per cluster:} 
Our platform will provide the user with well-organized and easily accessible information in a way that can facilitate the analysis of a forum and its identified clusters.
For example, Table~\ref{tab:clustsummary} provides a bird's-eye view of the clustering decomposition and the relative sizes.
Our web platform, we will have clickable links that one can follow to drill deeper into entities of interest.
Table~\ref{tab:1result} demonstrates another view that we would like to provide: all the columns, except the last, are populated automatically. The event explanation may be more difficult to achieve in general, though in some cases, starting from the list of the most dominant \textit{cluster keywords} (50 most important words in the cluster) can provide significant information. For example, one  such cluster talks about the outbreak of SimpleLocker, and the term ``SimpleLocker" is the second most frequent keyword in its \textit{cluster keywords}. 

%\miii{In para below: Flip the order: start with what we provide Top-k most indicative threads: .... sure professor --- BTW This is GREAT and we should highlight it. It is really cool! Thanks professor. All learnt from u!! Not allowed to make comments like this! :-) :-)}

\miii{I would suggest you come up with a name for this view: "storyline view" or Thread-Summary - TimePrint : for "thumbprint in time",  or something}

\miii{Keep here mostly he algorithmic part, specific things about the result, move them to next section:
The goal here is to make it sound automatic and hands free: find dominant topic(s), report the top-k threads that (a) related to the topic and (b) are "important"(?).}

\risul{ However, to further enhance the profiling of a cluster, we develop a systematic and easily interpretable method to identify the {\it k} most indicative  threads (as a representation of event/s) in the cluster. To achieve this, for each cluster, we create the document corpus considering the \textit{title} of each thread as ``document'' to train a LDA Bag-of-Words model \cite{sharma2017survey}. Then we extract the topics from the corpus where number of topics is equal to the number of threads in the cluster and number of words in each topic is equal to the average number of  words in the titles after standard preprocessing. Note that a topic is represented as a weighted list of words. Then we calculate the \% of topics a document is about (\textit{topic scores} for each document) and from there we assign each document a topic depending on the highest \textit{topic score}. In the next phase, we find the the distribution of the number of documents per topic and choose the \textit{dominant topics}. \textit{dominant topics} is the most representative topics' set representing at least 70\% of the documents. Finally, we report {\it k} [default=5] documents({\it titles}) having highest \textit{topic scores} for each of the \textit{dominant topics} in a story-line (non-decreasing timeline) manner demonstrated in Fig. \ref{fig:event_report}. We find that one topic, ransomware, represents 81\% of the {\it titles}. So, we report top 5 {\it titles} based on highest \textit{topic scores} for the ``ransomware'' topic in a sorted timeline fashion.
}


\end{comment}

==> arxiv-RECTEN (2)/0045-evaluation.tex <==
\section{Evaluation of \algo}
\label{sec:evaluation}
In the absence of proper ground truth for evaluation, we create synthetic tensors and apply \algo on them. We  show the effectiveness of our method by applying it on five real datasets as well discussed at {\it Application Results and Observations} Section. However, since \algo is a multi-modal hierarchical soft clustering method and there is a lack of ground truth, it becomes inherently hard and challenging to perform certain tasks including (i) labeling the extracted clusters, (ii) finding suitable evaluation metrics, and (iii) finding suitable comparison methods. We discuss these challenges in the following subsections.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,height=5cm]{fig/allsyncluster.png}
    \caption{Injected non-hierarchical pattern/clusters of different Types in our Synthetic tensor.}
    \label{fig:flatsynthetic}
\end{figure}

\subsection{Synthetic Tensor Construction}
\label{subsec:synthetictensor}
To evaluate \algo, we construct synthetic tensors and demonstrate the effectiveness of \algo in finding both hierarchical and non-hierarchical clusters. We describe the injection of both non-hierarchical and hierarchical clusters in synthetic tensors below.

{\bf A. Injecting non-hierarchical clusters in Synthetic Tensor.}
%\label{subsec:flatsynthetictensor}
We inject some non-hierarchical patterns in the form of clusters in a synthetic tensor demonstrated in Fig. \ref{fig:flatsynthetic}. We consider a 3-mode synthetic zero-tensor,$S$, with dimension $300\times 300 \times 30$ which is reasonable enough to emulate realistic patterns. Lets assume the modes are $A$, $B$, and $C$. $a_i, b_j, c_k$ are indices along modes $A$, $B$, and $C$. To imitate different types of overlapping and non-overlapping non-hierarchical clusters present in the data, we inject the following clusters in $S$ shown in Fig. \ref{fig:flatsynthetic}:

{\it a. SSD cluster pattern.} We insert three {\it SSD} cluster patterns, $P_1-P_3$, in $S$. These clusters have {\bf S}ame $a_i$'s, {\bf S}ame $b_j's$, but {\bf D}ifferent $c_k$'s. {\it b. SDS cluster pattern.} 3 {\it SDS} clusters, $P_4-P_6$, inserted; {\bf S}ame $a_i$'s, , {\bf D}ifferent $b_j$'s, {\bf S}ame $c_k's$. {\it c. DSS cluster pattern.} 3 clusters, $P_7-P_9$, inserted; {\bf D}ifferent $a_i$'s, {\bf S}ame $b_j$'s, {\bf S}ame $c_k's$. {\it d. DDD cluster pattern.} 3 clusters, $P_{10}-P_{12}$, inserted; {\bf D}ifferent $a_i$'s, {\bf D}ifferent $b_j$'s, {\bf D}ifferent $c_k's$. {\it e. DDS cluster pattern.} 3 clusters, $P_{13}-P_{15}$, inserted; {\bf D}ifferent $a_i$'s, {\bf D}ifferent $b_j$'s, {\bf S}ame $c_k's$. {\it f. DSD cluster pattern.} 3 clusters, $P_{16}-P_{18}$, inserted; {\bf D}ifferent $a_i$'s, {\bf S}ame $b_j$'s, {\bf D}ifferent $c_k's$. {\it g. SDD cluster pattern.} 3 clusters, $P_{19}-P_{21}$, inserted; {\bf S}ame $a_i$'s, {\bf D}ifferent $b_j$'s and {\bf D}ifferent $c_k$'s. 


A total of 21 cluster patterns have been injected in $S$ which works as ground truth for the evaluation of \algo. However, to emulate the realistic patterns, we also follow some rules while injecting the cluster patterns. For instance, each pattern has a clustroid $\eta$. The patterns are formed with entities within $d$ Manhattan distance dispersion and $\rho$ concentration (entities/pattern). There are 8 overlapping patterns in $DDD$, $DDS$, $DSD$, and $SDD$ types. We regulated the pattern size and density by varying $d$ and $\rho$. The domain of each entity in each cluster pattern is a Gaussian distribution, $G(\mu=10,\sigma=3)$.

{\bf B. Injecting hierarchical cluster in synthetic tensor.} The goal here is to generate a time-evolving synthetic tensor with 3D realistic hierarchical patterns in it. We achieve this goal by following the steps below.

First, we inject 2D self-similar hierarchical patterns in the base slice (slice 0) of the synthetic tensor. Next, we emulate a time-varying tensor by making stack of the copies of the base slice but with substantial changes at each time slice. We follow the simplest but realistic approach borrowing the ideas from \cite{leskovec2010kronecker} and \cite{guigoures2012triclustering} to construct this synthetic tensor. 

In more detail, we inject a hierarchical pattern utilizing Kronecker Multiplication of order three ($K_3$ adjacency matrix) \cite{leskovec2010kronecker} in the base slice (dimension 125X125) demonstrated in Fig. \ref{fig:kronecker}. The values of ``x'' in this Figure are drawn from a Gaussian distribution, $G(\mu=10,\sigma=3)$ and the white  places are all zeros. Next, we copy the base slice and make a stack of ten of these copies to emulate the time-evolving hierarchical pattern. To achieve substantial changes at each time slice, we randomly choose two zero-valued data points from each of the randomly chosen ten leaf clusters ($K_1$) and replace those with values from the above-mentioned Gaussian distribution. In this way, we can achieve a time-evolving synthetic tensor (dimension 125X125X10) with hierarchical structures in it as ground truth. In tree view, this synthetic tensor yields a total of 30 hierarchical clusters in two different levels (5 at level 1 and 25 more at level 2). These 30 clusters act as ground truth for evaluating \algo. We want to show that \algo is capable of identifying the clusters at their respective levels.  To show the effectiveness of \algo against noise, we also add positive Gaussian noise $G(\mu=0,\sigma=1)$ in randomly chosen $n\%$ of the entities at each time slice. We discuss the effect of the noise on the performance of \algo below in this Section. 

\begin{figure}[t]
    \centering
    \includegraphics[ width=\linewidth, height=2.75cm]{fig/kroneckernew.png}
    \caption{Example of Generation of Kronecker adjacency matrix $K_3$ for the base slice where $K_3 = K_2 \otimes K_1$ and $K_2 = K_1 \otimes K_1$. $\otimes$ is the Kronecker Multiplication operator.}
    \label{fig:kronecker}
\end{figure}
 
%Our next goal is to evaluate \algo based on how efficiently it can reveal these 21 cluster patterns as well as setting some model parameters empirically.

\subsection{Evaluation Metrics}
\label{subsec:eval_metrics}

Evaluating the clustering methods is always hard and challenging, especially hierarchical multi-aspect soft clustering. Previous methods \cite{luu2011approach, rand1971objective, zhang1989simple} suggested the use of performance metrics: Total Purity, Rand Index, and Tree Edit Distance in such case. We now briefly discuss these metrics below.

{\bf A. Total Purity. }We use the metric {\bf Total Purity}({\it TP}) to evaluate \algo \cite{luu2011approach}. It is measured on a scale of 0-1 where {\it TP=1} means perfect clustering and {\it TP=0} means no clustering at all. In our case, {\it TP=1} means no impurity i.e. each entity is in the cluster of similar kind.

We formally define a measure of clustering quality that is based on labeling information. Let L represents the set of labels (for non-hierarchical synthetic tensor $|L|=21$). Let $l(x)$ be the true label ($C_1-C_{21}$) of point $x$.
The label of a cluster, $C_i$, is the true label of the majority of points in that cluster, denoted by
$$l(C_i) = argmax_{b\in L}|{x \in C_i| l(x) = b}|$$
The impurity of a cluster is the proportion of points whose label differs from the labels of their cluster. 

{\it Definition 1. The total impurity ($TI$) of a clustering algorithm $A$, which yields a set cluster patterns $C$, is defined as:}

$$ TI(A) = \frac{1}{|C|}\sum_{i=1}^{|C|} \frac{\sum {x\in C_i| l(x) \neq l(C_i)}}{|C_i|}$$

In our case, $C$ is the set of cluster patterns yielded in the output of \algo. Thus, Total Purity of \algo is defined as:

$$TP(\algo)= 1 - TI(\algo)$$

{\bf B. Rand Index. } The Rand Index (RI) \cite{rand1971objective} computes a similarity measure between two clusterings by considering all pairs of samples and counting pairs that are assigned in the same or different clusters in the predicted and true clusterings. RI is ensured to have a value close to 0.0 for total random clustering and exactly 1.0 when the clusterings are identical. Given a set, S, of n elements and two clustering algorithms, X and Y, to compare, the formula to calculate RI is:

$$RI = \frac{a+b}{\binom{n}{2}}$$

where a is the number of pairs of elements in S that are in the same cluster in X and in the same cluster in Y. b is the number of pairs of elements in S that are in the different clusters in X and in the different clusters in Y. In our case, n denotes the total number of non-zero elements in the synthetic tensor. For ease of evaluation and comparison, we set the regularizer penalty term $\lambda$ to zero and we study the effect of $\lambda$ later in this Section.

{\bf C. Tree Edit Distance.} The hierarchical structures injected in our synthetic tensor can be viewed as a tree and the output of \algo can be viewed as the same as well. Therefore, to show that \algo does capture the same/similar tree structure, we evaluate \algo using another metric, Tree Edit Distance (TED) \cite{zhang1989simple}. TED between two labeled trees, $T_1$ and $T_2$, is the number of insertion, renaming and deletion operation needed to map exactly one tree onto another. The lower the TED, the better the clustering algorithm w.r.t. ground truth. 


\subsection{Parameter Tuning }
\label{subsec:eval}
We set the values of different parameters of \algo empirically by applying it on the synthetic tensors. We utilize TP and RI  evaluation metrics to do this. The results are discussed below.  

{\bf a. Effect of $\epsilon$.} Choosing the right $\epsilon$ is crucial for \algo. Very small $\epsilon$ can yield no meaningful pattern whereas very large $\epsilon$ can eliminate significant amount of information from the tensor. So, the goal is to find a sweet region where we can unravel meaningful patterns with least amount of deletion. Fig. \ref{fig:evsmetrics} demonstrates that $\epsilon=[4,8]\%$ is our sweet region where we achieve maximum performance based on both metrics, TP and RI, for both non-hierarchical and hierarchical cluster extraction from synthetic tensors.

\begin{figure}[t]
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/epsilon_flat.png}
        \caption{Non-hierarchical clustering.}%\reminder{From V: I understand that the abbreviation to A, T, P etc is good for brevity, but the figure is hard to just simply glance at (which many reviewers will), so maybe it would be a good idea to spell those words out}}
    \label{fig:evsmetricsflat}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/epsilon_hierarchy.png}
        \caption{Hierarchical clustering.}
    \label{fig:evsmetricshierarchical}
    \end{subfigure}
    ~
    
    \caption{$\epsilon$ vs. TP and RI ($k=15$,$\lambda,n=0$). 
    }
    \label{fig:evsmetrics}
    \vspace{-2mm}
\end{figure}


{\bf b. Effect of $k$.}
Another crucial parameter of \algo is $k$ which determines when to stop our recursive factorization. Very low $k$ yields in small factorized clusters breaking down the pattern to even more parts (value of performance metrics close to 1) whereas very high value of $k$ will preserve multiple convoluted patterns in a single cluster (value of performance metrics far away from 1). Fig. \ref{fig:kvsmetrics} exhibits that, for our synthetic tensors, both hierarchical and non-hierarchical, $k=[14,18]\%$ is our sweet region where we achieve reasonably high performance from \algo based on both TP and RI performance metrics. Moreover, setting $k=15, \epsilon=6$, and $\lambda=0.8$, we find that \algo is able to find 20 clusters in level 1, and 3 clusters in level 2 from the non-hierarchical synthetic data. The algorithm would perform ideally if it could extract all 21 non-hierarchical clusters in level 1. Similarly, \algo captures 6 clusters at level 1, 25 clusters at level 2 and 1 clusters at level 3 whereas ideal performance would be identifying 5 clusters at level 1 and 25 clusters at level 2 from hierarchical synthetic data. This suggests the effectiveness of \algo in identifying hidden clusters from data. 

\begin{figure}[t]
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/k_flat.png}
        \caption{Non-hierarchical clustering.}%\reminder{From V: I understand that the abbreviation to A, T, P etc is good for brevity, but the figure is hard to just simply glance at (which many reviewers will), so maybe it would be a good idea to spell those words out}}
    \label{fig:kvsmetricsflat}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/k_hierarchy.png}
        \caption{Hierarchical clustering.}
    \label{fig:kvsmetricshierarchical}
    \end{subfigure}
    ~
    
    \caption{$k$ vs. TP and RI ($\epsilon=6$,$\lambda,n=0$). 
    }
    \label{fig:kvsmetrics}
    \vspace{-2mm}
\end{figure}


{\bf c. Effect of $\lambda$. }
\begin{figure}[t]
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/lambdavstp.png}
        \caption{$\lambda$ vs. TP.}%\reminder{From V: I understand that the abbreviation to A, T, P etc is good for brevity, but the figure is hard to just simply glance at (which many reviewers will), so maybe it would be a good idea to spell those words out}}
    \label{fig:lambdavstp}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4cm,width=4.5cm]{fig/noisenvstp.png}
        \caption{$n$ vs. TP.}
    \label{fig:nvstp}
    \end{subfigure}
    ~
    
    \caption{Effect of $\lambda$ and $n$ ($k=15$,$\epsilon=6$). 
    }
    \label{fig:lambdaandn}
    \vspace{-2mm}
\end{figure}
The sparsity regularizer penalty term, $\lambda$, is used to filter out the noisy data points while decomposition. If $\lambda=0$, then there will be no filtration at all. One key difference of \algo with other clustering algorithms is that \algo also offers clustering with only key elements by increasing $\lambda$. But very high value of $\lambda$ can yield clusters with high cohesiveness but minimal information. Fig. \ref{fig:lambdavstp} demonstrates the effect of $\lambda$ on the performance of \algo. Empirical result suggests that setting the value of $\lambda$ to 0.8 can yield maximum performance with reasonable information preserved.

{\bf d. Effect of noise percentage, $n$. } 
We analyze the performance of \algo in the presence of noise and find that \algo can offer reasonable performance for noisy data. Fig. \ref{fig:nvstp} demonstrates the performance of \algo in extracting patterns from both hierarchical and non-hierarchical synthetic tensors in the presence of noise. We observe a sharp drop ``knee" in Fig. \ref{fig:nvstp} which suggests that \algo can produce reasonable outputs for up to $n=20\%$ data noise.

{\bf e. Discussion on $d, \rho, \mu, \sigma$}
We also analyze the performance of \algo by varying dispersion $d$, concentration $\rho$, and data value distribution parameters ( $\mu$ and $\sigma$). We find that \algo offers good performance for different combinations of these parameters as well. We omit the results here due to space limitations. 
%{\bf c. Randomly selection, biased probability inversely proportional, biased probability proportional  vs. TI}

%{\bf d. Levels vs. TI}

%{\bf f. $d$ vs. TI}

%{\bf g. $\rho$ vs. TI}

%{\bf i. $\sigma$ vs. TI}

%{\bf e. Levels vs. Number of clusters identified - original percentage, missed percentage, repeated percentage}

%{\bf h. Base algorithm without Regularization, Base algorithm with Regularization, \algo without Regularization, and \algo with Regularization vs. $\lambda$ vs. TI}



\subsection{Comparison with state-of-the-art methods}
\label{subsec:comparison}


To the best of our knowledge, we are the first to propose a method to extract hierarchical multi-modal clusters from multi-modal data using tensor decomposition. State-of-the-art methods find clusters from data represented in 2D matrix format whereas we find clusters from multi-modal data (tensor). Therefore, comparing results from two different kinds of data and cluster representation becomes inherently difficult. 

We try to compare the results with other widely-used and state-of-the-art methods anyway. To do this, we use four comparison methods including (i) widely-used basic Ward's method for Agglomerative Hierarchical Clustering Algorithm (AHC\_ward) \cite{ward1963hierarchical}, (ii) state-of-the-art frequency-based Agglomerative Hierarchical Clustering Algorithm (AHC\_freq) \cite{madheswaran2017improved}, (iii) local cores-based Hierarchical Clustering Algorithm (DLORE-DP) \cite{cheng2020dense}, and (iv) \algo without hierarchy (RecTen\_WH). We apply \algo as well as the above-mentioned Comparison Algorithms to extract structures from both the hierarchical and non-hierarchical synthetic tensors and compare their performance. 




Now, as a desperate attempt to compare the Comparison Algorithms, applied on data represented in 2D matrix, with \algo, applied on 3D tensor, we follow a tricky way. We compare the performance results from Comparison Algorithms applied on 2D slice $i$ of the synthetic tensors with performance results from \algo applied on 3D sub-tensor constructed from slice 0 to $i$. The comparison results are depicted in Fig. \ref{fig:comparisontp} and \ref{fig:comparisonted}. We find that \algo underperforms than others except RecTen\_WH for the base slice $i=0$. DLORE-DP actually produces better result than any of the other methods up to slice 2. But  as $i$ increases more and new non-zero entities are added on the slices, \algo outperforms all the other Comparison Algorithms. Fig. \ref{fig:comparisonted} demonstrates the performance of \algo for hierarchical structures discovery compared to other methods in terms of TED performance metrics. Note that the lower the TED is, the better the performance is. Similar to hierarchical pattern discovery, \algo does better than the Comparison Algorithms in finding non-hierarchical clusters as well. We omit this similar result due to space limitations.


==> arxiv-RECTEN (2)/0050-results.tex <==
\section{Application Results and Observations}
\label{sec:results}


\begin{figure}[t]
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4.5cm,width=4.5cm]{fig/comparisontp.png}
        \caption{Performance comparison of \algo in terms of TP.}%\reminder{From V: I understand that the abbreviation to A, T, P etc is good for brevity, but the figure is hard to just simply glance at (which many reviewers will), so maybe it would be a good idea to spell those words out}}
    \label{fig:comparisontp}
    \end{subfigure}
    ~
    \begin{subfigure}{0.48\columnwidth}
    \includegraphics[height=4.5cm,width=4.5cm]{fig/comparisonted.png}
        \caption{Performance comparison of \algo in terms of TED.}
    \label{fig:comparisonted}
    \end{subfigure}
    ~
    
    \caption{Performance comparison of \algo and our Comparison Algorithm for hierarchical cluster discovery. ($k=15$,$\epsilon=6,\lambda=0.8$). 
    }
    \label{fig:comparison}
    \vspace{-2mm}
\end{figure}

We provide proof of the effectiveness of \algo by finding interesting hierarchical clusters from five different real datasets, discussed in {\it Datasets} Section. The findings that we report here can help a security analyst mostly to a great deal. We discuss the findings below.


{\bf a. Results from security forums. } We construct a 3D tensor, $T$, by capturing the interaction of users with different threads at different weekly discretized times. Each element, $T(i,i,k)$ of the input tensor captures the interaction (in terms of the number of posts) of user $i$ with thread $j$ at  discretized week \textit{k} or zero in the absence of such interaction. We then fed the input tensor, $T$m to \algo. We find a total of 101 clusters from three security forums (41 from OC, 27 from HTS, and 33 from EH) arranged in hierarchical format (maximum depth 4). 

Upon investigating the cluster contents from OC forum, we find a cluster at level 1 revolving around Ransomware related discussion. The discussion started at Dec 2015 and further instigated in Feb 2016 (observed from the time dimension of the identified cluster) which mirrors the outbreak of SimpleLocker ransomware at that time. The detected cluster actually indicated the early warning of the coming ransomware disaster around the world. However, upon further investigation of that cluster by going one level down, we identified 12 threads containing 34 sellers of the decryption tools. By diving deep into the next level further, we identify a famous company, MDS, also selling decryption tools in this underground market.

Investigating one of the identified clusters at level 1 from HTS forum, we identify a bunch of threads by user {\it DoSman} offering free trial of his attack tools. Diving deep into the next level, we find posts related to selling DOS attack tools and phishing tools. EH forum also hides interesting clusters. For example, we identify {\it VandaDGod}, an expert Linux hacker, shared a popular tutorial series of hacking in Kali Linux in Nov 2017. Going one step down, we spot clusters related to `Hacking into Banks' and `Hacking Routers'. We find a series of posts to appoint new members for hacking into banks by {\it VandaDGod} in the next level. A simple internet search reveals that notorious hacker {\it VandaTheGod} is accused of hacking several government sites. This bears the indication that \algo does capture meaningful clusters.

{\bf b. Results from gaming forums. } Following the strategy similar  to security forums, we get a total of 233 clusters from MPGH organized in 6 levels (max depth of the output hierarchy tree is 6). We find clusters related to gaming strategies as well as some very peculiar and interesting clusters. For example, we identify a big cluster at level one revolving around different scamming and hacking related objections. Next level of this cluster comprises of clusters revolving around online gaming account scamming and `Romance Scamming'. It seems that in some online games where users can chat among themselves, scammers chat with female users to win their trust and scam for money. Also, we spot clusters related to searching for experienced hackers after a painful defeat in a game.  These surprising findings indicate that online gaming forums are being a new potential source of security threats.

{\bf c. Results from GitHub dataset. } Similar to security forums, we construct a 3D tensor for GitHub dataset as well. Each element, $T(i,i,k)$, of the input tensor captures the interaction (in terms of total number of create, fork, comment and contribution performed) of author $i$ with repository $j$ at  discretized week \textit{k} or zero in the absence of such interaction. Applying \algo on this tensor, we extract a total of 79 clusters in 4 levels (max depth 4). An interesting cluster contains Windows related malware in the first level and the next level contains Windows related ransomware. These clusters formed mainly in Jan 2016 when ransomware was spreading worldwide and malicious authors started developing more ransomware in GitHub inspired by the attack success. \algo can help the security enforcement authorities to keep track of which and how malware are being developed and getting popularity over time.

{\bf Empirical results comparison with TimeCrunch. } TimeCrunch \cite{shah2015timecrunch} is also a tensor based tool to discover patterns but it extracts only six fixed types of temporal structures, for example, oneshot full/near clique, periodic full/near bipartite cores etc. We apply TimeCrunch on three security forum datasets and find a total of only 17 structures. All these 17 structures are captured in \algo as well. \algo actually captures a total of 101 clusters from these security forums which is neither too few nor too many to analyze the clusterized actionable information. Therefore, \algo strikes a balance between finding too few and too many clusters to analyze. We omit the detailed finding of TimeCrunch due to space limitations. 


{\bf Open-source for maximal impact. } Inspired by the success of \algo, we implement it in a tool format to help the research community. \algo tool can run with default parameter settings ($k=15$, $\epsilon=6, \lambda=0.8$) but any savvy end-user can optionally tune the parameters upon his/her needs and preferences. \algo provides clickable links on the output tree view by which the end-users can gauge through his/her cluster of interest and the contents of the clusters as well. 

{\bf Computational effort. } The computation required by \algo is not excessive. The average runtime for preparing the final hierarchical Tree view of the biggest forum with 100K posts, MPGH, takes only 2.39 minutes on average. %which is fast enough to provide end-user satisfaction.
% The runtime is averaged over applying \algo on a particular forum for five times. 
Our experiments were conducted on a
machine with 2.3GHz Intel Core i5 processor and 16GB RAM.
We use Python v3.6.3 packages to implement all the modules of \algo. 
We believe that the runtime can be reduced to seconds if we use more powerful hardware.
These results suggest that \algo scales reasonably well in practice.

==> arxiv-RECTEN (2)/006-related.tex <==
\section{Related Work}
\label{sec:related}

%\reminder{From V: If we are going for a full WWW paper, this is very little related work. We should definitely discuss other (non security forum approaches, e.g., https://dl.acm.org/citation.cfm?id=2743004 and also just show tha we have a spherical view of the entire area. I am worried that reviewers will complain that related work is limited if we leave it as is.}
%\miii{If we submit a two pager - related may not be necessary}


To the best of our knowledge, RecTen is the first of its kind to extract actionable hierarchical patterns from multi-aspect data. Our work is different from the following perspective: (i) it is unsupervised, (ii) it is applied on multi-aspect data, and (iii) it leverages tensor factorization in a recursive way. The related works can be divided into the following categories:

{\bf a. Discovering hierarchical structures using non tensor approach.}
Hierarchical structure discovery is a very common task in data mining. The algorithms that are being used mostly include but not limited to bottom-up Agglomerative Hierarchical Clustering, top-down Hierarchical k-means Clustering, and variations of these algorithms. The basic and widely used version of Agglomerative Hierarchical Clustering is Ward's method \cite{ward1963hierarchical}. Different variations of bottom-up Hierarchical Clustering are being used recently as well \cite{teffer2019adahash, mahalakshmi2020gibbs}. \cite{cheng2020dense} developed a local cores-based hierarchical algorithm for dataset with complex structures. Another work \cite{madheswaran2017improved} proposed an improved frequency-based agglomerative clustering algorithm for detecting distinct clusters on two-dimensional dataset. The application of these types of  bottom-up hierarchical extends but not limited to analyzing the sentiment of the people in different regions from  geo-location tagged twitter posts \cite{batarseh2018geo}, categorizing the  in-hospital fall reports of the patients \cite{liu2019exploring}, and document clustering \cite{lee2017hierarchical, zainol2017document}. Variations of Top-down hierarchical algorithm like hierarchical k-means is also being used in different domains ranging from modeling blast-produced vibration \cite{nguyen2019new} to large graph embedding \cite{nie2020unsupervised}. \cite{kuang2013fast} focuses on hierarchical document clustering leveraging non-negative matrix factorization. All the above-mentioned algorithms suffer from the same problem. These algorithms are applied on data represented in 2D matrix format. Therefore,  finding clusters in multi-modal data requires new strategy. The work of \cite{guigoures2012triclustering} focused on tri-clustering in time evolving graphs but did not utilize tensor factorization at all.   


%A recent effort of \cite{batarseh2018geo} looked into the geo-location tagged twitter posts and analyzed the sentiment of the people in different regions utilizing hierarchical clustering of the posts.

%Another effort of \cite{liu2019exploring} categorized the  in-hospital fall reports of the patients leveraging the hierarchical clustering.

%\cite{lee2017hierarchical} proposes a hierarchical document clustering approach utilizing the frequent itemsets (words) in the documents.

%\cite{zainol2017document} cauterizes the military peacekeeping documents using hierarchical clustering to extract meaningful information.


{\bf b. Recursive hierarchical use of tensors.} Although the recursive use of tensor is very rare, a very recent work of \cite{abdali2020hijod} introduces an embedding framework to detect fake news leveraging hierarchical tensor and matrix decomposition up to two levels. Though the authors call it a hierarchical model, it is completely different from our work because we use only tensor decomposition recursively. Another work \cite{wang2015towards} utilized recursive tensor decomposition for interactive topic hierarchy construction which is related but not actual recursive factorization like we do in this study.   



\textbf{c. Other tensor decomposition approaches and applications.}
Tensor decomposition is a well-studied area with a wide range of diverse applications and domains ~\cite{kolda2009tensor}, ~\cite{liu2019community}, \cite{papalexakis2015understanding}, \cite{rettinger2012context}. \cite{shah2015timecrunch} proposed TimeCrunch which focused on mining some fixed temporal patterns from time-evolving dynamic graphs. Although the output of TimeCrunch are clusters like \algo, they are not organized in hierarchy.  

Relatively recently tensor-based techniques have been used in social media analytics as well to answer various questions. For example, ~\cite{papalexakis2015understanding} have used Tensor Decomposition to understand the multilingual social networks in online
immigrant communities. Another work of ~\cite{liu2019community} focused on community evolution by analyzing a feature matrix obtained by Tensor Decomposition. ~\cite{rettinger2012context} proposed a model for relationship prediction in social networks using context-aware Tensor Decomposition. Another type of tensor- based work includes community assignment of nodes in multi-aspect graph \cite{gujral2018smacd}.
%and hierarchical topic modeling \cite{wang2015towards}.
We are not aware of any tensor-based multi-modal hierarchical pattern discovery algorithm. In our work, we adapted the CP decomposition \cite{kolda2009tensor, faber2003recent} to find the base clusters and then factorized the clusters recursively.








% {\bf d. Online forum analysis methods (with or without tensors). }

% \cite{cobo2011modeling, cobo2012using} propose the use of agglomerative hierarchical clustering to group the similar students according to their activities in discussion forums. 

% \cite{pascual2009exploring} introduces a visualization tool for exploring the discussion thread to understand the large amount of information in online discussion.

% \cite{seo2009online} shows that proper hierarchical thread structures that have been accurately annotated can lead to significant improvements in  search performance. 

% \cite{tarnpradab2017toward} adapts
% the hierarchical attention networks for sentence level thread summarization.





==> arxiv-RECTEN (2)/007-conclusion.tex <==
\section{Conclusion}

We propose, \algo,  an unsupervised-learning tensor-based approach to  systematically discover quality cluster patterns in a multi dimensional space. It has parameter-free settings as well as optionally parameter tuning capability.
We show the effectiveness of our approach by an extensive evaluation of the identified clusters from synthetic data as well as from five real datasets. 

\algo has three main advantages:
(a) it operates in an unsupervised way, 
(b) it generalizes well to both categorical and numerical multi-modal data and scales well for large dataset too,
and 
(c) in its tool version, it supports clickable Tree view to investigate the clusters further.

Our work is a step towards an automated unsupervised capability,
which can allow the data analysts and researchers to shift through the wealth of information that exists in massive multi-modal data.


%\miii{In references: the last name of the first author needs to appear!!!!}

==> arxiv-RECTEN (2)/009-Acknowledgment.tex <==
\section{Acknowledgment}
\label{sec:Acknowledge}

%\thanks {This work was supported by  DHS ST Cyber Security (DDoSD)  HSHQDC-14-R-B00017 grant and the Bourns College of Engineering at UC Riverside}
%Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the funding parties.
 {%The authors thank the anonymous reviewers for their useful comments.
This material is based upon work supported by DHS ST Cyber Security (DDoSD)  HSHQDC-14-R-B00017 grant. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of 
%the National Science Foundation or other 
the funding institutions.}

==> arxiv-RECTEN (2)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> arxiv-RECTEN (2)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
